An agent-based model of an endangered population of the Arctic fox from Mednyi Island

Artificial Intelligence techniques such as agent-based modeling and probabilistic reasoning have shown promise in modeling complex biological systems and testing ecological hypotheses through simulation. We develop an agent-based model of Arctic foxes from Medniy Island while utilizing Probabilistic Graphical Models to capture the conditional dependencies between the random variables. Such models provide valuable insights in analyzing factors behind catastrophic degradation of this population and in revealing evolutionary mechanisms of its persistence in high-density environment. Using empirical data from studies in Medniy Island, we create a realistic model of Arctic foxes as agents, and study their survival and population dynamics under a variety of conditions.

==> Makefile <==
# $Id: Makefile,v 1.7 2003/06/22 09:23:35 m Rel $

NAME=soul
ARCHNAME=$(NAME).tar.gz
ARCHIVE=$(NAME).dtx Makefile $(NAME).txt $(NAME).ins
MAKEIDXOPT=
DVIPSOPT=#-Pcmz -Pamz
DEP=$(NAME).sty

all: $(NAME).sty $(NAME).ps

print: $(NAME).ps
	psbook $(NAME).ps|psnup -2|psselect -e|lpr
	@ echo -n revert paper stack and hit return
	@ read key
	psbook $(NAME).ps|psnup -2|psselect -o -r|lpr

ps: $(NAME).ps

%.ps: %.dvi
	dvips $(DVIPSOPT) $< -o $@

hyper: $(NAME).dtx $(NAME).sty
	pdflatex "\relax\let\makehyperref\active\input $(NAME).dtx"

$(NAME).pdf: $(NAME).dtx $(NAME).sty
	pdflatex $(NAME).dtx

archive:
	@ tar -czf $(ARCHNAME) $(ARCHIVE)
	@ echo $(ARCHNAME)

clean: 
	rm -f $(NAME).{log,toc,lot,lof,idx,ilg,ind,aux,blg,bbl,dvi,ins,out}

distclean: clean
	rm -f $(NAME).{ps,sty,pdf} $(ARCHNAME)


REFWARN = 'Rerun to get cross-references'
LATEXMAX = 5

%.dvi: %.dtx $(DEP)
	latex $< ; true
	RUNS=$(LATEXMAX); \
	while [ $$RUNS -gt 0 ] ; do \
		if grep $(REFWARN) $*.log > /dev/null; \
		then latex $< ; else break; fi; \
		RUNS=`expr $$RUNS - 1`; \
	done

$(NAME).sty: $(NAME).ins soul.dtx
	tex $(NAME).ins

$(NAME).ins:
	latex $(NAME).dtx


